Geometry-Based Data Generation

Many generative models attempt to replicate the density of their input data. However, this approach is often undesirable, since data density is highly affected by sampling biases, noise, and artifacts. We propose a method called SUGAR (Synthesis Using Geometrically Aligned Random-walks) that uses a diffusion process to learn a manifold geometry from the data. Then, it generates new points evenly along the manifold by pulling randomly generated points into its intrinsic structure using a diffusion kernel. SUGAR equalizes the density along the manifold by selectively generating points in sparse areas of the manifold. We demonstrate how the approach corrects sampling biases and artifacts, while also revealing intrinsic patterns (e.g. progression) and relations in the data. The method is applicable for correcting missing data, finding hypothetical data points, and learning relationships between data features.

==> Background.tex <==
Given a large high dimensional data set $\myvec{X}={\myvec{x}_1,...,\myvec{x}_N}\in{\mathbb{R}}^{D \times N}$ we assume that the data lies on some lower dimensional manifold $\cal{M}$. We aim to generate a set of new points $\myvec{Y}={\myvec{y}_1,...,\myvec{y}_M}\in{\mathbb{R}}^{D \times M}$ along the manifold $\cal{M}$. Our goal is to generate the point at sparse regions of $\myvec{X}$ such that the density of points in the final dataset $\myvec{Z}=\myvec{X} \cup \myvec{Y}$ is approximately uniform. 

Based on the manifold assumption we must first learn the intrinsic relations based on the samples from the manifold $M$. Learning the structure of the underlying manifold $\cal{M}$ is achieved using dimensionality reduction algorithms. Existing methods such as Multidimensional Scaling (MDS)
\cite{MDS}, Local Linear Embedding \cite{LLE}, Laplacian Eigenmaps
\cite{belkin2002laplacian} (LE) and Diffusion Maps (DM) \cite{lafon:DM} aim to reduce the complexity of the data while maintaining the important underlying structures and patterns. Diffusion Maps has been demonstrated effective for learning the underlying manifold in various fields. Some examples of DM based applications are presented in \cite{lafon2006data,liu2012learning,lindenbaum2015musical}. We first describe the steps required for extracting the diffusion based embedding.

==> Density.tex <==
\label{sec:sparse}
The MGC diffusion operator $\hat{\myvec{P}}$ defined in Eq. \ref{eq:Pmgc} is weighted by a sparsity measure $\hat{s}(i),i=1,...,N$. By design, we want $\hat{s}(i)$ to be large at sparse regions of $\cal{M}$. Thus, the MGC operator $\hat{\myvec{P}}$ will consist large values where $\hat{s}(i)$ is large. The sparsity measure, therefor, will uplift the probabilities of new points to locate at the sparse regions of $\cal{M}$.

We propose to compute a sparsity measure $\hat{s}(i)$ based on an estimate of the density $d(i)$ at each point. Kernel density estimators (KDE's) \cite{seaman1996evaluation,scott1985averaged,gine2002rates} are a popular and simple choice for estimating the density of high dimensional points. In the following, we describe simple KDE for computing the density at each point $\hat{d}(i),i=1,...,N,$ followed by the sparsity $\hat{s}(i)$. We note that any other approach that increases the weights for sparse regions could be useful.\\
%In this subsection we describe options for high dimensional density and sparsity measures.\\
{\bf{Kernel Density Estimation (KDE)}}\\
The proposed approach is not very sensitive to the accuracy of the density estimation, therefor, we use a simple estimation based on the kernel $\myvec{K}$  (described in Eq. \ref{GKernel}).
The decaying property of the radial basis function $\myvec{K}$ is used for measuring the number of adjacencies for each point. To do this, we compute the kernel with a constant bandwidth. Based on the kernel $\myvec{K}$, we estimate the density using the degree at each node. The KDE is defined by
\begin{equation} \label{eq:density}
K_{DE}(\myvec{x}_i) \defeq \hat{d}(i)=\sum_j exp\left( {-\frac{||\myvec{x}_i-\myvec{x}_j||^2}{2\sigma^2}  }\right),i=1,...,N,
\end{equation} by setting $\sigma^2=\text{mean} [ \underset{i,i\neq j}{\min} (||\myvec{x}_i-\myvec{x}_j||^2)]$ the kernel captures the variation of density along $\myvec{X} \subset \cal{M}$.\\
{\bf{Sparsity Measure}}\\
The sparsity measure $\hat{s}(i),i=1,...,N$ (appears in Eq. \ref{eq:mgc}) is designed to uplift the weights of the diffusion process around sparse regions of $\myvec{X} \subset \cal{M}$. We define the sparsity measure using the following equation:
\begin{equation} \label{eq:sparsity1}
\hat{s}(i)\defeq \frac{1}{\hat{d}(i)},i=1,...,N.
\end{equation}
Clearly $\hat{s}(i) \geq 0,i=1,...,N$, as the density $\hat{d}(i)$ at each point is non-negative (see Eq. \ref{eq:density}).


%{\bf{K-NN based density estimation}}
%The K-Nearest Neighbors method could also be applied for estimating the density of points. A simple approach would be to take the average distance from the first $K$ neighbors, and define the density as its inverse. This is defined by the following two steps. 

==> DensityEqualization.tex <==


The amount of points $\hat{\ell}(i)$ (step 4 in Algorithm \ref{alg:DataGeneration}) generated around each $\myvec{x}_i$ affects the distribution of points in $\myvec{Y}_1$. Here we present a method for approximating the number of points $\hat{\ell}(i)$ required for equalizing the distribution of points. By equalizing we mean that the density of generated points over $\cal{M}$ is uniform.
Given a biased data set our goal is to generate more points at sparse regions to balance the non-uniform density of $\myvec{X}$. To do this we have proposed to draw $\hat{\ell}(i)$ points around each point $\myvec{x}_i,i=1,...,N$ from ${\cal{N}}(\myvec{x}_i,\myvec{\Sigma}_i)$ (as described in Algorithm \ref{alg:DataGeneration}). The following proposition provides the ``correct'' number of points $\hat{\ell}(i),i=1,...,N$ required to balance the density over the manifold my equalizing the degrees $\hat{d}(i)$ (Eq. \ref{eq:deg}).
\begin{proposition} \label{prop}
For each point $\myvec{x}_i\in \cal{M} \backslash \partial{\cal{M}}$ the expectation value of the degree $\hat{d}(i)$ is constant if the number of points generated is given by
\begin{equation}
\hat{\ell}(i) = \lfloor \det(\myvec{\Sigma}^{-1}_i + \frac{\myvec{I}}{2\sigma^2})^{0.5}  \det(\myvec{\Sigma}_i )^{0.5} [{\max(\hat{d}(\cdot))-\hat{d}(i)}] \rfloor,
\end{equation}
where $\hat{d}(i)$ is the degree value at point $\myvec{x}_i$, $\sigma^2$ is the bandwidth of the kernel $\myvec{K}$ (Eq. \ref{GKernel}) and $\myvec{\Sigma}_i$ is the covariance of the Gaussian designed for generating new points (as described in Algorithm \ref{alg:DataGeneration}).   

\end{proposition}

\begin{proof}
Given $\myvec{x}_i \in \mathbb{R}^D,i=1,...,N$, the degree at point $\myvec{x}_i$ is defined in Eq. \ref{eq:deg}. SUGAR (Algorithm \ref{alg:DataGeneration}) generates $\hat{\ell}(i)$ points around $\myvec{x}_i$ from a Gaussian distribution $N(\myvec{x}_i,\myvec{\Sigma})$. After generating $\hat{\ell}(i)$ points, the degree at point $\myvec{x}_i$ is defined as
\begin{equation} \label{eq:Nkde_Full}
\hat{d}(i) =\sum^N_{j=1} e^ {-\frac{||\myvec{x}_i-\myvec{x}_j||^2}{2\sigma^2}  }  + \sum^{\hat{\ell}(i)}_{\ell=1} e^{-\frac{||\myvec{x}_i-\myvec{y}^i_{\ell}||^2}{2\sigma^2}  } .\end{equation}
In order to equalize the distribution, we require that the expectation of the degree be independent of $x_i$, thus, we set $\mathrm{E} \Big[ \hat{d}(i) \Big] =\text{C},i=1,...,N$, where $\text{C}$ is a constant that will be addressed later in the proof. Further, we notice that the first term in the right hand side of Eq.~$\ref{eq:Nkde_Full}$ can be substituted by $\hat{d}(i)$, while the second term is a sum of $\hat{\ell}(i)$ random variables. For simplicity, we assume at this point that the points generated around $\myvec{x}_i$ have negligible effect on the $\hat{d}(j)$ at point $j \neq i$. We note that this assumption should hold with proper choices of $\sigma$ and $\myvec{\Sigma}_i,i=1,...,N$. By substituting the constant $C$, the term $\hat{d}(i)$, and using the independence assumption, the expectation of Eq.~\ref{eq:Nkde_Const} can be written as
\begin{equation} \label{eq:Nkde_Const}
\text{C}-\hat{d}(i) =\mathrm{E} \Big[  \sum^{\hat{\ell}(i)}_{\ell=1} e^{-\frac{||\myvec{x}_i-\myvec{y}^i_{\ell}||^2}{2\sigma^2}  } \Big].\end{equation}
Then, since the variables $\myvec{y}^i_{\ell}$ are i.i.d., then the right hand side of Eq.~\ref{eq:Nkde_Const} becomes
\[ \hat{\ell}(i)  \mathrm{E} \Big[ e^{-\frac{||\myvec{x}_i-\myvec{y}^i||^2}{2\sigma^2}  }\Big]= \] 
\[\frac{\hat{\ell}(i)}{\det(2\pi \myvec{\Sigma}_i)^{1/2}} \int_{\mathbb{R}^D} { e^{-\frac{||\myvec{x}_i-\myvec{y}^i||^2}{2\sigma^2}  }} e^{- {(\myvec{x}_i-\myvec{y}^i)^T\myvec{\Sigma}^{-1}_i (\myvec{x}_i-\myvec{y}^i ) }} d \myvec{y}^i, \]
and then using a change of variables $\tilde{\myvec{y}}=\myvec{y}^i-\myvec{x}_i$, the integral simplifies to
\[ \frac{\hat{\ell}(i)}{\det(2\pi \myvec{\Sigma}_i)^{1/2}} \int_{\mathbb{R}^D} e^{- {(\myvec{x}_i-\myvec{y}^i)^T(\myvec{\Sigma}^{-1}_i + \frac{\myvec{I}}{2\sigma^2})(\myvec{x}_i-\myvec{y}^i ) }} d \myvec{y}^i= \]
\[ \frac{\hat{\ell}(i)} { \det(\myvec{\Sigma}^{-1}_i + \frac{\myvec{I}}{2\sigma^2})^{0.5}  \det(\myvec{\Sigma}_i )^{0.5}}, \]
where the final step is based on the integral of a Gaussian and a change of variables. Finally, we conclude that the estimator for the number of points $\hat{\ell}(i)$ is $\hat{\ell}(i)=\lfloor \det(\myvec{\Sigma}^{-1}_i + \frac{\myvec{I}}{2\sigma^2})^{0.5}  \det(\myvec{\Sigma}_i )^{0.5}[C- \hat{d}(i)] \rfloor $. By choosing $C=\max(\hat{d}(\cdot))$ we guarantee that $\hat{\ell}(i)\geq 0$ (which means that we are not removing points). In section \ref{sec:densexp} we demonstrate the proposed approach for density equalization. \qedhere

%The final estimator for the number of points is the quantized version of $\ell(i)$, explicitly $\hat{\ell}(i)= \lfloor \ell(i) \rfloor$.


\end{proof}

==> DensityExp.tex <==

In the following experiment we evaluate the proposed method for density equalization, as explained in Section~\ref{sec:dens}) based on Proposition~\ref{prop}, which provides a method for choosing the number of generated points $\hat{\ell}(i)$ at each region on the manifold. % This proposition is based on the assumption that the data is not sampled from the boundary of $\cal{M}$, therefore, to simplify the evaluation of the method we use a manifold without a boundary. 
We start by sampling a hundred points from a circle (see Fig.~\ref{fig:circ}) such that the highest density is at the origin ($\theta=0$) and the density decreases away from it. Figure~\ref{fig:circ1} shows each point $x_i$ colored by its degree $\hat{d}(i)$ (as defined in Eq.~\ref{eq:deg}). Figure~\ref{fig:circZt1} shows new points generated based on $\hat{\ell}(i)$ around each original point.
\begin{figure}[!htb]
\centering
\subfigure[]{\label{fig:circ1} \includegraphics[width=0.3\textwidth] {Circ1.png}}
\subfigure[] {\label{fig:circkde} \includegraphics[width=0.3\textwidth] {KDEcirc.png}}
\subfigure[] {\label{fig:ell_i} \includegraphics[width=0.3\textwidth] {Ell_i.png}}    
\caption{Density equalization demonstrated on a circle shaped manifold. \subref{fig:circ1} The original non-uniform samples of $\myvec{X}$. \subref{fig:circkde} The degree value $\hat{d}(i)$ at each point $\myvec{X}_i,i=1,...,100$. \subref{fig:ell_i} The number of generated points $\hat{\ell}(i),i=1,...,100$.}
\end{figure}
  
We then apply SUGAR and estimate the CDF of $\myvec{X}$ and $\myvec{Z}$ based on a projection of the points to the first coordinate. We note that the resulting distribution shown in blue is approximately a density of a standard uniform CDF as shown in red in Fig.~\ref{fig:circdens}. The variance of the degree $\hat{d}(\cdot)$ drops from 0.45 to 0.03, yet another indication of the improved density of points.

\begin{figure}[!htb]
\centering
\subfigure[] {\label{fig:circZt0} \includegraphics[width=0.3\textwidth] {CircZt0.png}}
\subfigure[] {\label{fig:circZt1} \includegraphics[width=0.3\textwidth] {CircZt1.png}}
\subfigure[] {\label{fig:circdens} \includegraphics[width=0.3\textwidth] {DensityCirc.png}} 
\caption{Density equalization demonstrated on a circle shaped manifold. \subref{fig:circZt0} The original points $\myvec{X}$ (black asterisks) and set of new generated points $\myvec{Y}_0$ (blue circles). \subref{fig:circZt1} The final set of points $\myvec{Z}$, original points $\myvec{X}$ (black asterisks) and set of new generated points $\myvec{Y}_t$ (blue circles). In this example only one diffusion time step is required (i.e. $t=1$). \subref{fig:circdens} An estimation of the CDF before (black asterisks) and after (blue circles) applying the SUGAR compared to the CDF of a standard uniform distribution. }
\label{fig:circ}
\end{figure} 

  
  
  
    
    
    
